Personalization of Web Search During the 2020 US Elections

Search engines play a central role in routing political information to citizens. The algorithmic personalization of search results by large search engines like Google implies that different users may be offered systematically different information. However, measuring the causal effect of user characteristics and behavior on search results in a politically relevant context is challenging. We set up a population of 150 synthetic internet users ("bots") who are randomly located across 25 US cities and are active for several months during the 2020 US Elections and their aftermath. These users differ in their browsing preferences and political ideology, and they build up realistic browsing and search histories. We run daily experiments in which all users enter the same election-related queries. Search results to these queries differ substantially across users. Google prioritizes previously visited websites and local news sites. Yet, it does not generally prioritize websites featuring the user's ideology.

==> fig/tab_serp_similarity.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Apr 09, 2022 - 06:37:54 PM
\begingroup 
\small 
\begin{tabular}{@{\hspace{5pt}}l@{\hspace{5pt}}c} 
\toprule 
 & \multicolumn{1}{c}{Dependent variable:} \\ 
\cmidrule(rr){2-2} 
 & Search results similarity (Jaccard) \\ 
\midrule  
\\[-2.1ex] Browsing similarity\n(Jaccard) & 0.018$^{*}$ \\ 
  & (0.010) \\ 
 \addlinespace 
 Search similarity\n(Jaccard) & 0.011 \\ 
  & (0.009) \\ 
 \addlinespace 
 Same city & 0.024$^{***}$ \\ 
  & (0.007) \\ 
 \addlinespace 
 Time difference\n(in h) & $-$0.006$^{***}$ \\ 
  & (0.001) \\ 
 \addlinespace 
\midrule  
Observations & 1,773,605 \\ 
R$^{2}$ & 0.448 \\ 
\bottomrule 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\endgroup 


==> tab/tab_SM_serp_similarity.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Jun 09, 2021 - 10:17:27 PM
\begin{table}[!htb] \centering 
  \caption{Differences in search results pages} 
  \label{tab:SM_serp_similarity} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\emph{Dependent variable:} SERP similarity} \\ 
\cline{2-5} 
\\[-1.8ex] & \multicolumn{2}{c}{Jaccard} & \multicolumn{2}{c}{RBO} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Same ideology & $-$0.0002 & 0.0001 & $-$0.0002 & $-$0.0001 \\ 
  & (0.001) & (0.001) & (0.001) & (0.0004) \\ 
  & & & & \\ 
 Same city & 0.011$^{**}$ & 0.010$^{***}$ & 0.010$^{**}$ & 0.007$^{***}$ \\ 
  & (0.005) & (0.002) & (0.005) & (0.001) \\ 
  & & & & \\ 
 Same browser language & 0.055$^{***}$ & 0.037$^{**}$ & 0.041$^{***}$ & 0.018$^{*}$ \\ 
  & (0.010) & (0.017) & (0.009) & (0.010) \\ 
  & & & & \\ 
 Time difference (days) & $-$0.006$^{***}$ & $-$0.007$^{***}$ & $-$0.005$^{***}$ & $-$0.005$^{***}$ \\ 
  & (0.001) & (0.002) & (0.001) & (0.001) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Search term FE & X & X & X & X \\ 
Sample & Organic results & Topstories & Organic results & Topstories \\ 
Observations & 8,956,604 & 1,673,737 & 8,956,604 & 1,673,737 \\ 
R$^{2}$ & 0.453 & 0.308 & 0.542 & 0.337 \\ 
Adjusted R$^{2}$ & 0.453 & 0.308 & 0.542 & 0.337 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{5}{p{12cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by search term and synthetic user pair. The unit of observation is search term-user pair. The dependent variable is the Rank-Biased Overlap
                 computed from different SERP parts (organic search results, top stories, ads) of SERPs presented to a user $i$ and a user $j$ when using the same search term. 
                    The explanatory variable \emph{`Same ideology'} is equal to 1 if users i and j have the same political ideology (either D, R, or apolitical) and 0 otherwise. 
                    The explanatory variable \emph{`Same city'} is equal to 1 if users i and j are located in the same city and 0 otherwise. 
                    The explanatory variable \emph{`Same browser language'} is equal to 1 if users i and j use the same language setting in their web browser and 0 otherwise. 
                    The explanatory variable \emph{`Time difference (days)'} is the absolute time difference between the searches of i and j, measured in (fraction of) days. Since some search terms have been used on several days 
                    throughout the entire duration of the experiment and since we are comparing all searches of all bots using the same search term, the difference can be sevaral days in these comparisons.
                    If a bot pair issued the search on the same date in the same city, the searches were also usually issued within minutes of the same time of the day.
                    In all specifications we account for search term fixed effects (as some user pairs might have used the same search term more than once). The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_familiarity.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, May 04, 2021 - 10:03:45 PM
\begin{table}[!htb] \centering 
  \caption{SERPs Familiarity and Previous Page Visits} 
  \label{tab:familiarity} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{Dependent variable: SERP Familiarity Score (organic search results)} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{serp\_familiarity\_score} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 $\# Visits$ & 0.022$^{***}$ & 0.018$^{***}$ & 0.017$^{***}$ & 0.018$^{***}$ & 0.017$^{***}$ & 0.025$^{***}$ \\ 
  & (0.002) & (0.001) & (0.001) & (0.001) & (0.001) & (0.002) \\ 
  & & & & & & \\ 
 Democrat & $-$0.038$^{***}$ & $-$0.023$^{**}$ & $-$0.019$^{*}$ &  &  &  \\ 
  & (0.010) & (0.010) & (0.010) &  &  &  \\ 
  & & & & & & \\ 
 Republican & 0.004 & 0.005 & 0.006 &  &  &  \\ 
  & (0.009) & (0.010) & (0.010) &  &  &  \\ 
  & & & & & & \\ 
 Days elapsed &  &  &  &  & 0.001$^{***}$ & 0.0004$^{**}$ \\ 
  &  &  &  &  & (0.0002) & (0.0002) \\ 
  & & & & & & \\ 
 $\# Searches$ &  &  &  &  &  & $-$0.013$^{***}$ \\ 
  &  &  &  &  &  & (0.002) \\ 
  & & & & & & \\ 
 Constant & 0.110$^{***}$ &  &  &  &  &  \\ 
  & (0.009) &  &  &  &  &  \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Search term FE &  & X & X & X & X & X \\ 
Synthetic user FE &  &  &  & X & X & X \\ 
Date FE &  &  & X &  &  &  \\ 
Observations & 28,209 & 28,209 & 28,209 & 28,209 & 28,209 & 28,209 \\ 
R$^{2}$ & 0.412 & 0.528 & 0.558 & 0.619 & 0.620 & 0.653 \\ 
Adjusted R$^{2}$ & 0.412 & 0.527 & 0.555 & 0.616 & 0.617 & 0.651 \\ 
F statistic (full model) &6581.214 & 449.094 & 196.758 & 209.264 & 209.612 & 240.853 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{7}{p{12cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by date and synthetic user. The unit of observation is user-SERP. Only SERPs resulting from neutral searches (all users search the same) are considered.The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user
                 is configured as having liberal (conservative) political preferences (with apolitical synthetic users in the reference category). The variable \emph{Days elapsed} measures the number of days passed since the begin of the experiment (mid-October 2020) at the time the search query was issued.
                           The varible $\# Searches$ measures the total number of times user $i$ has previously (previous to the current neutral search query) used familiar domains shown in the SERP as a search term (e.g., googling for breitbart.com). The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_familiarity_topstories.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, May 04, 2021 - 10:03:47 PM
\begin{table}[!htb] \centering 
  \caption{SERPs Familiarity (Top Story Component) and Previous Page Visits} 
  \label{tab:familiarity_topstories} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\toprule \\
 & \multicolumn{6}{c}{Dependent variable: SERP Familiarity Score (top story component)} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{serp\_familiarity\_score} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\midrule \\
 $\# Visits$ & 0.021$^{***}$ & 0.018$^{***}$ & 0.018$^{***}$ & 0.019$^{***}$ & 0.019$^{***}$ & 0.031$^{***}$ \\ 
  & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.003) \\ 
  & & & & & & \\ 
 Democrat & $-$0.043$^{**}$ & $-$0.031$^{*}$ & $-$0.028 &  &  &  \\ 
  & (0.017) & (0.017) & (0.017) &  &  &  \\ 
  & & & & & & \\ 
 Republican & 0.035$^{**}$ & 0.038$^{**}$ & 0.039$^{***}$ &  &  &  \\ 
  & (0.014) & (0.015) & (0.015) &  &  &  \\ 
  & & & & & & \\ 
 Days elapsed &  &  &  &  & 0.001$^{***}$ & 0.001$^{*}$ \\ 
  &  &  &  &  & (0.0004) & (0.0003) \\ 
  & & & & & & \\ 
 $\# Searches$ &  &  &  &  &  & $-$0.019$^{***}$ \\ 
  &  &  &  &  &  & (0.003) \\ 
  & & & & & & \\ 
 Constant & 0.116$^{***}$ &  &  &  &  &  \\ 
  & (0.012) &  &  &  &  &  \\ 
  & & & & & & \\ 
\midrule \\ 
Search term FE &  & X & X & X & X & X \\ 
Synthetic user FE &  &  &  & X & X & X \\ 
Date FE &  &  & X &  &  &  \\ 
Observations & 8,887 & 8,887 & 8,887 & 8,887 & 8,887 & 8,887 \\ 
R$^{2}$ & 0.414 & 0.483 & 0.514 & 0.576 & 0.579 & 0.636 \\ 
Adjusted R$^{2}$ & 0.413 & 0.479 & 0.505 & 0.566 & 0.568 & 0.627 \\ 
F statistic (full model) &2088.093 & 130.743 & 57.009 & 56.195 & 56.438 & 71.371 \\ 
\bottomrule \\
%\multicolumn{7}{p{12cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by date and synthetic user. The unit of observation is user-SERP. Only SERPs resulting from neutral searches (all users search the same) are considered.The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user
%                 is configured as having liberal (conservative) political preferences (with apolitical synthetic users in the reference category). The variable \emph{Days elapsed} measures the number of days passed since the begin of the experiment (mid-October 2020) at the time the search query was issued.
%                           The varible $\# Searches$ measures the total number of times user $i$ has previously (previous to the current neutral search query) used familiar domains shown in the SERP as a search term (e.g., googling for breitbart.com). The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_jaccard_rbo_all_neutral.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Apr 27, 2021 - 12:39:04 PM
\begin{table}[!htbp] \centering 
  \caption{Differences in search results pages} 
  \label{} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{3}{c}{SERP Jaccard Index} & \multicolumn{3}{c}{SERP Rank Biased Overlap} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Same ideology & 0.002 & 0.001 & 0.010$^{***}$ & 0.001 & 0.001 & 0.006$^{**}$ \\ 
  & (0.001) & (0.002) & (0.002) & (0.001) & (0.001) & (0.002) \\ 
  & & & & & & \\ 
 Same city & 0.053$^{***}$ & 0.030$^{***}$ & 0.105$^{***}$ & 0.036$^{***}$ & 0.022$^{***}$ & 0.136$^{***}$ \\ 
  & (0.015) & (0.005) & (0.028) & (0.012) & (0.005) & (0.035) \\ 
  & & & & & & \\ 
 Same browser language & 0.121$^{***}$ & 0.100$^{***}$ & 0.024$^{***}$ & 0.097$^{***}$ & 0.059$^{***}$ & 0.036$^{***}$ \\ 
  & (0.012) & (0.011) & (0.006) & (0.013) & (0.012) & (0.010) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
SERP component & Organic results & Top stories & Ads & Organic results & Top stories & Ads \\ 
Search term FE & X & X & X & X & X & X \\ 
Observations & 632,334 & 105,992 & 74,822 & 632,334 & 105,992 & 74,822 \\ 
F statistic (full model) &10669.896 & 2208.505 & 1106.344 & 16268.693 & 5039.504 & 1455.615 \\ 
R$^{2}$ & 0.542 & 0.560 & 0.341 & 0.643 & 0.744 & 0.405 \\ 
Adjusted R$^{2}$ & 0.542 & 0.560 & 0.341 & 0.643 & 0.744 & 0.405 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{7}{p{14cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by search term and synthetic user pair. The unit of observation is search term-user pair. In specifications 1-4 (5-8) the dependent variable is the Jaccard index (Rank Biased Overlap)
                 computed from different SERP parts (organic search results, top stories, ads) of SERPs presented to a user i and a user j when using the same search term. 
                    The explanatory variable \emph{`Same ideology'} is equal to 1 if users i and j have the same political ideology (either D, R, or apolitical) and 0 otherwise. 
                    The explanatory variable \emph{`Same city'} is equal to 1 if users i and j are located in the same city and 0 otherwise. 
                    The explanatory variable \emph{`Same browser language'} is equal to 1 if users i and j use the same language setting in their web browser and 0 otherwise. 
                    In all specifications we account for search term fixed effects (as some user pairs might have used the same search term more than once). The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_rbo_all_neutral.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, May 13, 2021 - 03:39:20 PM
\begin{table}[!htb] \centering 
  \caption{Differences in search results pages} 
  \label{tab:rbo_all_neutral} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{SERP Rank-Biased Overlap} \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 Same ideology & 0.0004 & 0.001 & 0.005$^{**}$ \\ 
  & (0.001) & (0.001) & (0.002) \\ 
  & & & \\ 
 Same city & 0.035$^{***}$ & 0.022$^{***}$ & 0.135$^{***}$ \\ 
  & (0.012) & (0.005) & (0.035) \\ 
  & & & \\ 
 Same browser language & 0.097$^{***}$ & 0.054$^{***}$ & 0.036$^{***}$ \\ 
  & (0.013) & (0.011) & (0.010) \\ 
  & & & \\ 
 Same date & 0.016$^{***}$ & 0.033$^{***}$ & 0.022 \\ 
  & (0.006) & (0.012) & (0.017) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
SERP component & Organic results & Top stories & Ads \\ 
Search term FE & X & X & X \\ 
Observations & 632,334 & 105,992 & 74,822 \\ 
R$^{2}$ & 0.644 & 0.747 & 0.406 \\ 
Adjusted R$^{2}$ & 0.644 & 0.746 & 0.406 \\ 
F statistic (full model) &16104.755 & 5031.424 & 1419.504 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{4}{p{9cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by search term and synthetic user pair. The unit of observation is search term-user pair. The dependent variable is the Rank-Biased Overlap
                 computed from different SERP parts (organic search results, top stories, ads) of SERPs presented to a user $i$ and a user $j$ when using the same search term. 
                    The explanatory variable \emph{`Same ideology'} is equal to 1 if users i and j have the same political ideology (either D, R, or apolitical) and 0 otherwise. 
                    The explanatory variable \emph{`Same city'} is equal to 1 if users i and j are located in the same city and 0 otherwise. 
                    The explanatory variable \emph{`Same browser language'} is equal to 1 if users i and j use the same language setting in their web browser and 0 otherwise. 
                    The explanatory variable \emph{`Same date'} is equal to 1 if users i and j issued the Google search on the same day (this is per design of the experiment in slightly over 70% of the observations the case).
                    If a bot pair issued the search on the same date in the same city, the searches were also usually issued within minutes of the same time of the day.
                    In all specifications we account for search term fixed effects (as some user pairs might have used the same search term more than once). The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_serp_ideology.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Jun 10, 2021 - 12:44:11 PM
\begin{table}[!htb] \centering 
  \caption{Ideological leaning of search results pages (organic results)} 
  \label{tab:serp_ideology} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{Dependent variable: SERP ideology score} \\ 
\cline{2-9} 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
\hline \\[-1.8ex] 
 Democrat & $-$0.064 & $-$0.063 & 0.204$^{*}$ & $-$0.172 & $-$0.069 & $-$0.225 & $-$0.153$^{**}$ & $-$0.178$^{***}$ \\ 
  & (0.050) & (0.099) & (0.115) & (0.165) & (0.128) & (0.243) & (0.068) & (0.032) \\ 
  & & & & & & & & \\ 
 Republican & $-$0.008 & $-$0.094 & 0.011 & $-$0.289$^{***}$ & $-$0.325$^{***}$ & $-$0.207$^{***}$ & $-$0.345$^{***}$ & $-$0.227 \\ 
  & (0.056) & (0.083) & (0.107) & (0.059) & (0.117) & (0.004) & (0.089) & (0.138) \\ 
  & & & & & & & & \\ 
 Dem. city & $-$0.498 & $-$0.114 & 0.239 & 0.041 & 0.284 & 0.023 & 0.082 & $-$0.348 \\ 
  & (0.309) & (0.185) & (0.280) & (0.222) & (0.215) & (0.222) & (0.123) & (0.455) \\ 
  & & & & & & & & \\ 
 Rep. city & 0.336$^{*}$ & 0.108 & 0.459$^{**}$ & 0.320 & 0.494$^{***}$ & 0.303 & 0.016 & 0.499$^{***}$ \\ 
  & (0.170) & (0.103) & (0.222) & (0.340) & (0.174) & (0.212) & (0.043) & (0.183) \\ 
  & & & & & & & & \\ 
\hline \\[-1.8ex] 
Ideology measure & Robertson et al. & Bakshy et al. & Mturk & Budak & Allsides comm & Pew & MediaBias & Joint \\ 
\% domains in index & 83.87 & 49.02 & 56.66 & 21.71 & 39.07 & 39.07 & 30.73 & 54.84 \\ 
Language FE & X & X & X & X & X & X & X & X \\ 
Search term FE & X & X & X & X & X & X & X & X \\ 
Date of search FE & X & X & X & X & X & X & X & X \\ 
Observations & 25,644 & 25,644 & 25,644 & 25,644 & 25,644 & 25,644 & 25,644 & 25,644 \\ 
R$^{2}$ & 0.780 & 0.569 & 0.737 & 0.591 & 0.853 & 0.648 & 0.832 & 0.872 \\ 
F statistic (full model) &502.283 & 187.068 & 396.192 & 204.092 & 391.645 & 820.848 & 260.634 & 701.014 & 965.858 \\ 
Adjusted R$^{2}$ & 0.779 & 0.566 & 0.735 & 0.588 & 0.852 & 0.646 & 0.831 & 0.871 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{9}{p{18.5cm}}{\emph{Notes:} OLS regressions with robust standard errors three-way clustered by synthetic user, search term, and date of search. The unit of observation is the SERP. The dependent variable is the weighted average ideology of domains listed in the organic search results on a liberal-conservative
                 scale [-100,100] for different ideology indices measured for SERPs resulting from neutral searches (all users search the same).The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user is configured as having liberal (conservative) political preferences. The reference category is an apolitical synthetic user (no partisan browsing and search behavior). 
                     In all specifications we account for browser language setting fixed effects, search term fixed effects, and date of search fixed effects. The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_serp_ideology_all.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, May 13, 2021 - 11:39:59 PM
\begin{table}[!htb] \centering 
  \caption{Ideological leaning of search results pages} 
  \label{tab:serp_ideology_all} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{Dependent variable: SERP ideology score for component...} \\ 
\cline{2-5} 
\\[-1.8ex] & Organic results & Organic results (new) & Top stories & Top stories (new) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Democrat & $-$0.251$^{***}$ & $-$0.333$^{**}$ & 0.690 & 1.781$^{***}$ \\ 
  & (0.039) & (0.134) & (0.702) & (0.536) \\ 
  & & & & \\ 
 Republican & $-$0.228$^{*}$ & $-$0.190 & 0.450 & 1.397$^{*}$ \\ 
  & (0.137) & (0.117) & (0.453) & (0.769) \\ 
  & & & & \\ 
 Dem. city & $-$0.371 & $-$0.707$^{**}$ & 0.028 & $-$0.056 \\ 
  & (0.406) & (0.325) & (0.501) & (0.467) \\ 
  & & & & \\ 
 Rep. city & 0.457$^{**}$ & 0.531$^{***}$ & $-$0.966 & 0.242 \\ 
  & (0.175) & (0.170) & (0.853) & (1.083) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
\% domains in index & 84.74 & 84.74 & 92.16 & 92.16 \\ 
Language FE & X & X & X & X \\ 
Date of search FE & X & X & X & X \\ 
Observations & 28,963 & 28,963 & 8,584 & 8,584 \\ 
F statistic (full model) &1104.272 & 606.898 & 132.81 & 53.498 \\ 
R$^{2}$ & 0.883 & 0.805 & 0.744 & 0.540 \\ 
Adjusted R$^{2}$ & 0.882 & 0.804 & 0.739 & 0.530 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{5}{p{12cm}}{\emph{Notes:} OLS regressions with robust standard errors multiway clustered by synthetic user, search term, and date of search. The unit of observation is a SERP (either the organic search results or the top story component) resulting from a neutral search. 
                 The dependent variable is the weighted average ideology of domains listed in the organic search results, top story component, or ads component on a liberal-conservative
                 scale from -100 (consistently liberal) to 100 (consistently conservative) based on eight ideology indices (Robertson et al., Bakshy et al., Mturk, Budak, Allsides, Allsides community, Pew, MediaBias; all scaled to [-100, 100]). For each domain appearing in the corresponding SERP component,
                 we first compute the average ideological index, resulting in one value per search result list entry (or a missing value if the domain was not covered in any of the eight indices). The average ideology values are then multiplied by a 
                 weighing factor (defined as $\sqrt{N}$) in order to give observations based on more indeces more weight.
                 We then compute the average weighted ideological leaning as suggested in equations~\ref{eq:ideology} and \ref{eq:ideology_weight} with $p=0.9$ based on these values.
                 Only SERPs resulting from neutral searches are considered (all users searched for the same).
                 The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user is configured as having liberal (conservative) political preferences. 
                 The reference category is an apolitical synthetic user (no specific partisan browsing and search behavior, only random visits to the top 40 most visited US websites).
                The explanatory variable \emph{Dem. city} (\emph{Rep. city}) is equal to 1 if a substantial majority of voters in the synthetic user's city/location is Democrat (Republican).
                 The reference category are 'purple' cities (comparatively) close to a 50\% Democrat -- 50\% Republican voter share. For example, San Francisco, Washington DC, and Boston are considered Dem. cities, Detroit, Houston and Phoenix 
                 are considered purple cities, and Omaha, Witchita, and Oklahoma City are considered Rep. cities.
                           In all specifications we account for browser language setting fixed effects and date of search fixed effects. 
                           The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_serp_ideology_all_current.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, May 03, 2021 - 10:59:55 PM
\begin{table}[!htb] \centering 
  \caption{Ideological leaning of search results pages} 
  \label{tab:serp_ideology_all} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{Dependent variable: SERP ideology score for component...} \\ 
\cline{2-5} 
\\[-1.8ex] & Organic results & Organic results (new) & Top stories & Top stories (new) \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Democrat & $-$0.258$^{*}$ & $-$0.290 & 0.525 & 0.853$^{*}$ \\ 
  & (0.147) & (0.180) & (0.552) & (0.433) \\ 
  & & & & \\ 
 Republican & $-$0.023 & $-$0.028 & 0.415 & 0.759 \\ 
  & (0.193) & (0.194) & (0.440) & (0.480) \\ 
  & & & & \\ 
 Dem. city & $-$0.561$^{**}$ & $-$0.667$^{***}$ & 0.136 & $-$0.051 \\ 
  & (0.251) & (0.180) & (0.495) & (0.431) \\ 
  & & & & \\ 
 Rep. city & 0.363$^{*}$ & 0.570$^{***}$ & $-$0.350 & 0.240 \\ 
  & (0.196) & (0.145) & (0.619) & (0.548) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
\% domains in index & 84.74 & 84.74 & 92.16 & 92.16 \\ 
Language FE & X & X & X & X \\ 
Date of search FE & X & X & X & X \\ 
Observations & 28,963 & 28,963 & 8,584 & 8,584 \\ 
F statistic (full model) &326.311 & 163.302 & 68.021 & 47.551 \\ 
R$^{2}$ & 0.593 & 0.422 & 0.499 & 0.411 \\ 
Adjusted R$^{2}$ & 0.592 & 0.420 & 0.492 & 0.402 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{5}{p{12cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by synthetic user and date of search. The unit of observation is a SERP (either the organic search results or the top story component) resulting from a neutral search. 
                 The dependent variable is the weighted average ideology of domains listed in the organic search results, top story component, or ads component on a liberal-conservative
                 scale from -100 (consistently liberal) to 100 (consistently conservative) based on eight ideology indices (Robertson et al., Bakshy et al., Mturk, Budak, Allsides, Allsides community, Pew, MediaBias; all scaled to [-100, 100]). For each domain appearing in the corresponding SERP component,
                 we first compute the average ideological index, resulting in one value per search result list entry (or a missing value if the domain was not covered in any of the eight indices). The average ideology values are then multiplied by a 
                 weighing factor (defined as $\sqrt{N}$) in order to give observations based on more indeces more weight.
                 We then compute the average weighted ideological leaning as suggested in equations~\ref{eq:ideology} and \ref{eq:ideology_weight} with $p=0.9$ based on these values.
                 Only SERPs resulting from neutral searches are considered (all users searched for the same).
                 The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user is configured as having liberal (conservative) political preferences. 
                 The reference category is an apolitical synthetic user (no specific partisan browsing and search behavior, only random visits to the top 40 most visited US websites).
                The explanatory variable \emph{Dem. city} (\emph{Rep. city}) is equal to 1 if a substantial majority of voters in the synthetic user's city/location is Democrat (Republican).
                 The reference category are 'purple' cities (comparatively) close to a 50\% Democrat -- 50\% Republican voter share. For example, San Francisco, Washington DC, and Boston are considered Dem. cities, Detroit, Houston and Phoenix 
                 are considered purple cities, and Omaha, Witchita, and Oklahoma City are considered Rep. cities.
                           In all specifications we account for browser language setting fixed effects and date of search fixed effects. 
                           The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_serp_ideology_all_linh.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu May 13 23:39:59 2021
\begin{table}[ht]
\centering
\caption{Linear Hypothesis Tests (Table \ref{tab:serp_ideology_all})} 
\label{tab:serp_ideology_all_linh}
\begin{tabular}{llrr}
  \hline
Specification & Hypothesis & Chisq & Pr($>$Chisq) \\ 
  \hline
(1) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.04 & 0.84 \\ 
  (2) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 3.04 & 0.08 \\ 
  (3) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.13 & 0.72 \\ 
  (4) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.26 & 0.61 \\ 
  (1) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 2.94 & 0.09 \\ 
  (2) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 7.51 & 0.01 \\ 
  (3) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 2.19 & 0.14 \\ 
  (4) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 0.10 & 0.76 \\ 
   \hline
\end{tabular}
\end{table}



==> tab/tab_serp_ideology_all_linh_current.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon May  3 22:55:18 2021
\begin{table}[ht]
\centering
\caption{Linear Hypothesis Tests (Table \ref{tab:serp_ideology_all})} 
\label{tab:serp_ideology_all_linh}
\begin{tabular}{llrr}
  \hline
Specification & Hypothesis & Chisq & Pr($>$Chisq) \\ 
  \hline
(1) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 1.42 & 0.23 \\ 
  (2) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 3.64 & 0.06 \\ 
  (3) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.05 & 0.82 \\ 
  (4) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.07 & 0.79 \\ 
  (1) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 11.26 & 0.00 \\ 
  (2) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 29.50 & 0.00 \\ 
  (3) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 0.76 & 0.39 \\ 
  (4) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 0.34 & 0.56 \\ 
   \hline
\end{tabular}
\end{table}



==> tab/tab_serp_ideology_linh.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Jun 10 12:44:11 2021
\begin{table}[ht]
\centering
\caption{Linear Hypothesis Tests (Table \ref{tab:serp_ideology})} 
\label{tab:serp_ideology_linh}
\begin{tabular}{llrr}
  \hline
Specification & Hypothesis & Chisq & Pr($>$Chisq) \\ 
  \hline
(1) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.50 & 0.48 \\ 
  (2) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.39 & 0.54 \\ 
  (3) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 6.12 & 0.01 \\ 
  (4) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.34 & 0.56 \\ 
  (5) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 9.93 & 0.00 \\ 
  (6) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 30.45 & 0.00 \\ 
  (7) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 0.01 & 0.94 \\ 
  (8) & $\hat{\beta}_{Democrat}-\hat{\beta}_{Repuclican}=0$ & 24.48 & 0.00 \\ 
  (1) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 3.37 & 0.07 \\ 
  (2) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 6.17 & 0.01 \\ 
  (3) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 1.16 & 0.28 \\ 
  (4) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 1.06 & 0.30 \\ 
  (5) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 5.48 & 0.02 \\ 
  (6) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 192.97 & 0.00 \\ 
  (7) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 0.23 & 0.64 \\ 
  (8) & $\hat{\beta}_{Dem. city}-\hat{\beta}_{Rep. city}=0$ & 2.54 & 0.11 \\ 
   \hline
\end{tabular}
\end{table}



==> tab/tab_serp_ideology_topstories.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Jun 10, 2021 - 12:44:55 PM
\begin{table}[!htb] \centering 
  \caption{Ideological leaning of search results pages (topstories component)} 
  \label{tab:serp_ideology_topstories} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lcccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{8}{c}{Dependent variable: SERP topstories component ideology score} \\ 
\cline{2-9} 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
\hline \\[-1.8ex] 
 Democrat & 0.848$^{**}$ & 0.831$^{**}$ & 0.478 & 0.114 & 0.126 & 0.364 & 0.625 & 0.699 \\ 
  & (0.325) & (0.318) & (0.346) & (0.635) & (0.371) & (0.480) & (0.485) & (0.730) \\ 
  & & & & & & & & \\ 
 Republican & 0.332 & 0.029 & 0.425 & 0.529 & 0.249$^{*}$ & 0.502 & 0.925$^{*}$ & 0.447 \\ 
  & (0.219) & (0.234) & (0.271) & (0.533) & (0.149) & (0.336) & (0.530) & (0.472) \\ 
  & & & & & & & & \\ 
 Dem. city & 0.234 & $-$0.102 & 0.476 & $-$0.189 & $-$0.499 & $-$0.207 & $-$0.299 & $-$0.027 \\ 
  & (0.278) & (0.150) & (0.347) & (0.575) & (0.503) & (0.566) & (0.652) & (0.513) \\ 
  & & & & & & & & \\ 
 Rep. city & $-$0.134 & $-$0.275 & $-$0.303 & $-$0.507 & $-$0.442 & $-$0.008 & $-$1.032 & $-$1.021 \\ 
  & (0.354) & (0.425) & (0.412) & (0.658) & (0.346) & (0.661) & (0.655) & (0.888) \\ 
  & & & & & & & & \\ 
\hline \\[-1.8ex] 
Ideology measure & Robertson et al. & Bakshy et al. & Mturk & Budak & Allsides comm & Pew & MediaBias & Joint \\ 
\% domains in index & 91.86 & 71.98 & 70.72 & 32.74 & 53.19 & 53.19 & 41.86 & 66.48 \\ 
Language FE & X & X & X & X & X & X & X & X \\ 
Search term FE & X & X & X & X & X & X & X & X \\ 
Date of search FE & X & X & X & X & X & X & X & X \\ 
Observations & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 \\ 
R$^{2}$ & 0.612 & 0.597 & 0.589 & 0.590 & 0.622 & 0.601 & 0.598 & 0.720 \\ 
F statistic (full model) &73.818 & 69.531 & 67.103 & 67.341 & 63.224 & 77.068 & 70.528 & 69.664 & 120.655 \\ 
Adjusted R$^{2}$ & 0.603 & 0.589 & 0.580 & 0.581 & 0.614 & 0.592 & 0.589 & 0.714 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{9}{p{18.5cm}}{\emph{Notes:} OLS regressions with robust standard errors two-way clustered by synthetic user, search term, and date of search. The unit of observation is the SERP. The dependent variable is the weighted average ideology of domains listed in the top stories component on a liberal-conservative
                 scale [-100,100] for different ideology indices measured for SERPs resulting from neutral searches (all users search the same).The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user is configured as having liberal (conservative) political preferences. The reference category is an apolitical synthetic user (no partisan browsing and search behavior). 
                     In all specifications we account for browser language setting fixed effects, search term fixed effects, and date of search fixed effects. The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} \\ 
\end{tabular} 
\end{table} 


==> tab/tab_serp_ideology_topstories_notknown.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jul 27, 2021 - 11:33:36 AM
\begin{table}[!htb] \centering 
  \caption{Ideological leaning of search results pages (top stories component)} 
  \label{tab:serp_ideology_topstories_notknown} 
\scriptsize 
\begin{tabular}{@{\extracolsep{5pt}}lccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{9}{c}{Dependent variable: SERP (top stories component) ideology score (only new domains)} \\ 
\cline{2-10} 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)\\ 
\hline \\[-1.8ex] 
 Democrat & 1.213$^{**}$ & 0.993$^{*}$ & 1.638$^{***}$ & 2.448$^{***}$ & 0.466 & 1.871$^{***}$ & 1.090$^{***}$ & 1.844$^{***}$ & 1.826$^{***}$ \\ 
  & (0.547) & (0.533) & (0.491) & (0.837) & (0.419) & (0.649) & (0.301) & (0.543) & (0.564) \\ 
  & & & & & & & & & \\ 
 Republican & 0.011 & 0.196 & 1.091$^{***}$ & 2.186$^{***}$ & 0.224 & 1.335$^{**}$ & 0.991$^{***}$ & 1.449$^{*}$ & 1.446$^{*}$ \\ 
  & (0.404) & (0.582) & (0.351) & (0.584) & (0.337) & (0.562) & (0.254) & (0.810) & (0.768) \\ 
  & & & & & & & & & \\ 
 Dem. city & $-$0.716 & $-$0.425 & $-$0.319 & $-$0.565 & 0.489 & 0.108 & $-$0.080 & $-$0.094 &  \\ 
  & (0.430) & (0.559) & (0.744) & (0.773) & (0.403) & (0.879) & (0.349) & (0.455) &  \\ 
  & & & & & & & & & \\ 
 Rep. city & $-$0.779 & $-$0.053 & 0.996 & $-$0.511 & $-$0.136 & 1.029 & 0.242 & 0.250 &  \\ 
  & (0.708) & (0.845) & (0.863) & (1.081) & (0.586) & (1.023) & (0.530) & (1.121) &  \\ 
  & & & & & & & & & \\ 
 Share Rep. voters &  &  &  &  &  &  &  &  & 0.002 \\ 
  &  &  &  &  &  &  &  &  & (0.026) \\ 
  & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Ideology measure & Allsides & Bakshy et al. & Budak & MediaBias & Mturk & Pew & Robertson et al. & Joint & Joint \\ 
\% domains in index & 53.19 & 71.98 & 32.74 & 66.48 & 70.72 & 41.86 & 91.86 & 92.16 & 92.16 \\ 
Language FE & X & X & X & X & X & X & X & X & X \\ 
Search term FE & X & X & X & X & X & X & X & X & X \\ 
Date of search FE & X & X & X & X & X & X & X & X & X \\ 
Observations & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 & 8,327 \\ 
R$^{2}$ & 0.516 & 0.511 & 0.546 & 0.449 & 0.448 & 0.499 & 0.525 & 0.535 & 0.535 \\ 
Adjusted R$^{2}$ & 0.505 & 0.501 & 0.537 & 0.437 & 0.436 & 0.488 & 0.515 & 0.525 & 0.525 \\ 
\hline 
\hline \\[-1.8ex] 
%\multicolumn{10}{p{18.5cm}}{\emph{Notes:} OLS regressions with robust standard errors three-way clustered by synthetic user, search term, and date of search. The unit of observation is the SERP (topstories component). The dependent variable is the weighted average ideology of domains (not initially known by any of the synthetic users) listed in the top stories component on a liberal-conservative scale [-100,100] for different ideology indices measured for SERPs resulting from neutral searches (all users search the same). The explanatory variable \emph{Democrat} (\emph{Republican}) is equal to 1 if a synthetic user is configured as having liberal (conservative) political preferences. The reference category is a non-partisan synthetic user (no partisan browsing and search behavior). 
%The explanatory variable 'Share Rep. voters' is the share of Republican voters in the city where the synthetic user is located. In all specifications we account for browser language setting fixed effects, search term fixed effects, and date of search fixed effects. The statistical significance of coefficient estimates is indicated as follows: $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01.} 
\\ 
\end{tabular} 
\end{table} 


==> tab/tab_serp_ideology_userideology.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Apr 13, 2022 - 10:52:58 AM
\begin{tabular}{@{\hspace{5pt}}l@{\hspace{5pt}}cccc} 
\toprule 
 & \multicolumn{4}{c}{Dependent variable: search results ideology score} \\ 
\cmidrule(rr){2-5} 
 & Joint (new domains) & Joint (all domains) & \multicolumn{2}{c}{Local (new domains)} \\ 
 \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(rr){4-5}
 & (1) & (2) & (3) & (4)\\ 
\midrule  
\\[-2.1ex] Visited Sites Ideology & 0.002 & 0.001 & 0.001 & 0.021 \\ 
  & (0.004) & (0.004) & (0.003) & (0.014) \\ 
 \addlinespace 
 Dem. city & $-$0.540 & $-$0.452 & $-$0.558 & 0.004 \\ 
  & (0.358) & (0.370) & (0.372) & (0.241) \\ 
 \addlinespace 
 Rep. city & 0.676$^{***}$ & 0.587$^{***}$ & 0.530$^{***}$ & 0.420 \\ 
  & (0.196) & (0.181) & (0.129) & (0.494) \\ 
 \addlinespace 
\midrule  
Observations & 23,474 & 23,499 & 23,299 & 10,701 \\ 
R$^{2}$ & 0.760 & 0.777 & 0.793 & 0.830 \\ 
Adjusted R$^{2}$ & 0.758 & 0.775 & 0.791 & 0.827 \\ 
%Residual Std. Error & 9.388 (df = 23294) & 8.035 (df = 23319) & 10.012 (df = 23119) & 15.013 (df = 10544) \\ 
\bottomrule 
 \\ 
\end{tabular} 


==> tab/tab_serp_similarity.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Apr 09, 2022 - 07:09:24 PM
\medskip
\begingroup 
\footnotesize 
\begin{tabular}{@{\hspace{5pt}}l@{\hspace{5pt}}c} 
\toprule 
% & \multicolumn{1}{c}{Dependent variable:} \\ 
%\cmidrule(rr){2-2} 
Dependent variable: Search results similarity (JI) \\ 
\midrule  
\\[-2.1ex] Browsing similarity (JI) & 0.018$^{*}$ \\ 
  & (0.010) \\ 
 \addlinespace 
 Search similarity (JI) & 0.011 \\ 
  & (0.009) \\ 
 \addlinespace 
 Same city & 0.024$^{***}$ \\ 
  & (0.007) \\ 
 \addlinespace 
 Time difference (in h) & $-$0.006$^{***}$ \\ 
  & (0.001) \\ 
 \addlinespace 
\midrule  
Observations & 1,773,605 \\ 
R$^{2}$ & 0.448 \\ 
\bottomrule 
\end{tabular} 
\endgroup 

